Context-Aware Sentiment Forecasting via LLM-based Multi-Perspective Role-Playing Agents

User sentiment on social media reveals the underlying social trends, crises, and needs. Researchers have analyzed users' past messages to trace the evolution of sentiments and reconstruct sentiment dynamics. However, predicting the imminent sentiment of an ongoing event is rarely studied. In this paper, we address the problem of \textbf{sentiment forecasting} on social media to predict the user's future sentiment in response to the development of the event. We extract sentiment-related features to enhance the modeling skill and propose a multi-perspective role-playing framework to simulate the process of human response. Our preliminary results show significant improvement in sentiment forecasting on both microscopic and macroscopic levels.

==> Text/Preliminaries.tex <==
\section{Problem Formulation}
Text, as the written language distributed through different media, is an essential medium for communicating and expressing emotions~\cite{goldenberg2020digital}. OSN's prevalence allows people to communicate their feelings to the public in a timely way. Emotion dynamics for text messages can be studied retrospectively thanks to these digital footprints. Prospective emotion dynamics research would enhance social studies and public management, alleviating social crises when the spread of fear and anxiety is anticipated.

In light of this, we define the problem of \textbf{emotion dynamics forecast} to predict the evolution of emotion on OSN. It lies under the umbrella of emotion dynamics, which analyzes the trajectories, patterns, and regularities of emotional experiences. Emotion dynamics is affected by various interacting factors, including the individual and their environment. It could be harnessed to analyze the change in people's emotions through various expressions. Traditional emotion dynamics studies focus on fitting the evolution of one's emotion to the past outputted text. Emotion dynamics forecast is a prospective study to predict future emotional states. It could be evaluated on different scales, from individuals to a general crowd, according to different needs. A high individual accuracy rate is optimistic. When an event concerns a group of people more than others, predicting the group's emotional response would also gain a valuable understanding of group dynamics. 

For a prospective study, forecasting emotion dynamics needs to be both timely and concurrent with the development of an ongoing event. Unlike retrospective studies, where analysis occurs after the event has unfolded, the forecast must be generated before the event fully develops. Consequently, the forecasting process should be efficient and not time-consuming. It must utilize the available data from OSNs to perform real-time predictions, ensuring that insights are provided as the event progresses. The system requires minimal prerequisites, including the users' historical content, their follower-followee relationships, and the contexts of the event. These elements represent the essential individual and environmental interacting factors. Intuitively, on an individual level, the availability of more individual and environmental factors should enhance the accuracy of predictions. For a crowd, shared general characteristics can compensate for the absence of specific individual labels. However, in real-world applications, retrieving such labels is often challenging due to privacy concerns. Therefore, it is crucial to extract valuable information from OSN texts and environmental factors to effectively forecast user emotions.
%However, human evolution dynamics are extremely intricate. A highly accurate forecast rate is difficult to achieve. It is yet another valuable subject of research. Increasing the accuracy rate could enhance the understanding of OSN trends and help intervene in potential social crises in advance.

In this paper, the problem of \textbf{emotion dynamics forecast} is constrained to an unimodal approach, focusing solely on textual data. A more comprehensive emotion dynamics forecast might involve diverse modalities and measurements, including but not limited to voice, facial expressions, psychophysical signals, etc.  Expanding to a multimodal approach could significantly enhance the development of more personalized and nuanced human-machine interactions.

The forecast should revolve around a certain ongoing event $\mathcal{O}$, e.g. the Olympic Games. We can describe $\mathcal{O}$ with a short phrase, like hashtags or topics in OSN. As the event develops, the event contexts $\mathcal{E}_{t+1} = \{e_1, e_2, ..., e_{n}, e_{n+1}\}$ would update. It can be described with a few sentences in natural languages. 

\sloppy 
\begin{definition} \textbf{Emotion Dynamics Forecast}


Given a sequence of OSN comments $\mathcal{C}_t^u = \{c_1^u, c_2^u, \dots, c_n^u\}$ from a user $u$, the observed followee's commments $\mathcal{F}_t^u = \{ f_1^u, f_2^u, ..., f_n^u \}$, and the corresponding event contexts $\mathcal{E}_{t+1} = \{e_1, e_2, ..., e_{n}, e_{n+1}\}$ for an ongoing event $O$, the user's response $\sigma_{n+1}^u$ to the most recent update of event $e_{n+1}$ is predicted. The OSN comments $\mathcal{C}$, $\mathcal{F}$, and the contexts $\mathcal{E}$ evolve at real-time w.r.t. the development of the event. Therefore, the emotion dynamics forecast problem can be formulated as follows:
\begin{equation} 
\label{eqn: definition}
\begin{aligned} 
\sigma_{t+1}^u=f(\mathcal{C}_t^u, \mathcal{F}_t^u, \mathcal{E}_{t+1}).
\end{aligned}
\end{equation}
\end{definition}
It's important to note that an emotional response typically experiences a delay after the occurrence of the most recent event update. Namely, a user would post a comment $c$ only after the most recent context $e$ has occurred. This period of delay creates a fleeting window of opportunity for emotion dynamics forcast. 

